SiamMo: Siamese Motion-Centric 3D Object Tracking

Current 3D single object tracking methods primarily rely on the Siamese matching-based paradigm, which struggles with textureless and incomplete LiDAR point clouds. Conversely, the motion-centric paradigm avoids appearance matching, thus overcoming these issues. However, its complex multi-stage pipeline and the limited temporal modeling capability of a single-stream architecture constrain its potential. In this paper, we introduce SiamMo, a novel and simple Siamese motion-centric tracking approach. Unlike the traditional single-stream architecture, we employ Siamese feature extraction for motion-centric tracking. This decouples feature extraction from temporal fusion, significantly enhancing tracking performance. Additionally, we design a Spatio-Temporal Feature Aggregation module to integrate Siamese features at multiple scales, capturing motion information effectively. We also introduce a Box-aware Feature Encoding module to encode object size priors into motion estimation. SiamMo is a purely motion-centric tracker that eliminates the need for additional processes like segmentation and box refinement. Without whistles and bells, SiamMo not only surpasses state-of-the-art methods across multiple benchmarks but also demonstrates exceptional robustness in challenging scenarios. SiamMo sets a new record on the KITTI tracking benchmark with 90.1\% precision while maintaining a high inference speed of 108 FPS. The code will be released at https://github.com/HDU-VRLab/SiamMo.

==> Table/sparsity.tex <==
\begin{table}[t]
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|cc|cc}
\toprule[0.4mm]
\rowcolor{black!10}       &  & \multicolumn{2}{c|}{Kitti} & \multicolumn{2}{c}{Nuscenes} \\
\rowcolor{black!10} \multirow{-2}{*}{Method}       & \multirow{-2}{*}{Degrees} & Success    & Precision    & Success      & Precision     \\
\midrule
\multirow{2}{*}{M$^2$-Track}     & hard               & 53.0       & 67.0         & 52.1         & 60.9          \\
                              & medium              & 60.2       & 73.9         & 57.2         & 65.9          \\
\midrule
\multirow{2}{*}{\textbf{SiamMo(ours)}} & hard               & 64.8       & 75.7         & 64.1         & 72.5          \\
                              & medium              & 70.7       & 84.6         & 64.8         & 72.9         \\
\bottomrule[0.4mm]
\end{tabular}}
\caption{Robustness to the scenarios in sparse settings.}
\label{sparsity}
\end{table}
